Towards Identity-Aware Cross-Modal Retrieval: a Dataset and a Baseline

Recent advancements in deep learning have significantly enhanced content-based retrieval methods, notably through models like CLIP that map images and texts into a shared embedding space. However, these methods often struggle with domain-specific entities and long-tail concepts absent from their training data, particularly in identifying specific individuals. In this paper, we explore the task of identity-aware cross-modal retrieval, which aims to retrieve images of persons in specific contexts based on natural language queries. This task is critical in various scenarios, such as for searching and browsing personalized video collections or large audio-visual archives maintained by national broadcasters. We introduce a novel dataset, COCO Person FaceSwap (COCO-PFS), derived from the widely used COCO dataset and enriched with deepfake-generated faces from VGGFace2. This dataset addresses the lack of large-scale datasets needed for training and evaluating models for this task. Our experiments assess the performance of different CLIP variations repurposed for this task, including our architecture, Identity-aware CLIP (Id-CLIP), which achieves competitive retrieval performance through targeted fine-tuning. Our contributions lay the groundwork for more robust cross-modal retrieval systems capable of recognizing long-tail identities and contextual nuances. Data and code are available at https://github.com/mesnico/IdCLIP.

==> extended_related_works.tex <==
In recent years, vision-language models, and especially image-text matching methods, has gained significant attention, especially thanks to its immediate application in cross-modal retrieval scenarios. Many text-image matching methods adopt hinge-based triplet ranking loss with hard-negative mining. Early approaches utilized GRUs for text extraction \cite{faghri2018vse++}, later transitioning to Transformer encoders \cite{li2019visual,messina2022aladin,qu2020context,stefanini2021novel,wen2020learning}.
%
%The rise of Transformers in vision tasks \cite{dosovitskiy2020vit} has led to early-fusion models that process images and text jointly, treating image-text matching as a binary classification problem . Despite strong performance, these models are often computationally intensive for large-scale inference.
%
In contrast, late-fusion methods -- which stand against effective yet inefficient early-fusion methods \cite{beit3,li2021align,li2020oscar,lu2019vilbert,Su2020VL-BERT,zhang2021vinvl} -- process images and text separately and calculate similarity via a simple dot product \cite{messina2022aladin,sarafianos2019adversarial,radford2021learning,jia2021scaling}. Among these, CLIP \cite{radford2021learning} has become particularly influential for image-text matching and a strong backbone to solve many downstream vision-language tasks. %\cite{liu2023unleashing} proposes a model to find persons given textual descriptions but ignoring contextual information.
Despite their effectiveness in generic cross-modal retrieval, all of these methods cannot be employed directly to search for long-tail or out-of-distribution concepts unless largely fine-tuned. 

Most of the personalized vision-language research focused on personalized image generation. Gal et al. \cite{galimage} and Pang et al. \cite{pang2024cross} employed textual inversion to improve personalized feature learning, with variations in initialization methods. Wei et al. \cite{wei2023elite} and Gal et al. \cite{gal2023encoder} proposed encoder-based methods for efficient and accurate customization. Tewel et al. \cite{tewel2023key} introduced Perfusion, a mechanism for integrating multiple concepts while preventing overfitting, improving inference speed. Other approaches, such as Avrahami et al. \cite{avrahami2023break}'s multi-concept extraction from a single image, Chen et al. \cite{chen2024tailored}'s user history-based prompt rewriting, and Zeng et al. \cite{zeng2024jedi}'s fine-tuning-free method, contribute to advancing personalized text-to-image models. Despite these advances, our work focuses on attending to face identity, offering a different angle from object-specific personalization in prior studies.

Some works also started exploring personalized text-image retrieval. Cohen et al. \cite{cohen2022my} introduced a PerVL setup that leverages few-shot learning to reason about personalized concepts. Differently from our work, they update an already existing generic model, fine-tuning it on a small set of specific concepts. Yeh et al. \cite{yeh2023meta} tackled personalized video searches by learning instance-specific embeddings without requiring annotated data, enabling instance retrieval in personal videos through vision-language similarity.
The work most similar to our idea is \cite{korbar2022personalised} which introduce a method (\textit{CLIP-PAD}) and a dataset (\textit{Celebrities in Action}) for in-context person retrieval. Nevertheless, the proposed dataset collects only very famous actors that may be already present in the CLIP training dataset. We improve on their method CLIP-PAD by adding a targeted fine-tuning of the CLIP visual backbone for further enhance the fine-grained facial understanding abilities.


% \paragraph{Composed image-text retrieval}
% The proposed architecture is more similar to the ones performing composed image retrieval (CIR), in which a reference picture is used, together with a modification text, to find another picture more relevant to the given text.
% Vo et al. \cite{vo2019composing} first introduced CIR by proposing a residual-gating method to compose the image-text features, aiming to effectively integrate multimodal information. Subsequent works \cite{shin2021rtic,lee2021cosmo} further refined the CIR techniques, employing graph networks or decoupling image style and content.
% Recently, CLIP-based approaches have become prominent in CIR research. Baldrati et al. \cite{baldrati2022effective} demonstrated the effectiveness of combining out-of-the-box image-text features from CLIP using a combiner network. Later, they introduced a task-oriented fine-tuning step for the CLIP text encoder to achieve state-of-the-art performance \cite{baldrati2022conditioned}.
% The authors in \cite{agnolucci2024isearle,baldrati2023zero} further improved on the task to introduce the zero-shot CIR that does not require labeled datasets. 
%\cite{suo2024knowledge}

%TODO: forse anche questo transform and tell è rilevante
% "Transform and Tell: Entity-Aware News Image Captioning"
